Decision-support for the Masses by Enabling Conversations with Open Data

Open data refers to data that is freely available for reuse. Although there has been rapid increase in availability of open data to public in the last decade, this has not translated into better decision-support tools for them. We propose intelligent conversation generators as a grand challenge that would automatically create data-driven conversation interfaces (CIs), also known as chatbots or dialog systems, from open data and deliver personalized analytical insights to users based on their contextual needs. Such generators will not only help bring Artificial Intelligence (AI)-based solutions for important societal problems to the masses but also advance AI by providing an integrative testbed for human-centric AI and filling gaps in the state-of-art towards this aim.

==> background.tex <==
% --------------------
\section{ Conversation, Dialog and Chatbots}

Conversational interfaces (CI) traditionally refer to  automated systems that can engage with a user on one or more topics. They can be textual or speech-based dialog systems. There is  a long history of CIs going back to 1960s when they first appeared to answer questions or do casual conversation\cite{dialog-intro}. The term {\em dialog} is often interchangeably used with conversation in the context of textual conversation. 
A chatbot is an automated conversation agent, whether physical like robots or abstract like an avatar, that can not only interact with a person, but also  take actions on their behalf and get things done. One can talk to a chatbot or, if speech is not supported, type an utterance and get the system’s response.

In terms of conversation structure, a {\em dialog} is made up of a series of {\em turns}, where each turn is a series of {\em utterances} by one or more participants playing one or more {\em roles}. As examples, an on-line forum can have a single role of {\em users} while a customer support dialog may have the roles of {\em customer} and {\em support agent}.

For the rest of the paper, we will focus on a text-based agent that can interact with a human and also take actions on their behalf, if delegated. We will use the terms conversation interfaces (CIs), dialog agents and chatbots inter-changeably.



\subsection{Related Work}

There is a rich body of work on dialog analyses are often driven by advancement of speech and dialog systems \cite{mctear2002spoken}, focusing on developing NLP and machine learning methods to understand, predict and evaluate dialogs (e.g. \cite{young2013pomdp}).

[Add related work on learning dialog policies]

[Add related work on reasoning/ slot filling dialogs]
% In the example of customer support center, a user contacts a service center and enters into a dialog with a customer support agent. The participant roles here are that of a customer and an agent, and the roles inter-leave in every turn. On the other hand, in the example of online support, a person may raise an issue on a public portal and anyone may reply. 

[RADU to add some basic definitions and preliminaries -- not needed perhaps ?]

\cite{dialog-suitability}
% % --------------------
% \subsection{Example 1 - Finding Information from a Taxonomy}

% One popular category of user dialogs in business setting is inquiry of information that is organized in a taxonomy. For instance, a person wants to ask about a product on a company's site (e.g., {\em pliers} - product, job openings) but does not know which particular type. An example of taxonomy is
% United Nations Standard Products and Services Code (UNSPSC\footnote{https://www.unspsc.org/}), which {\em "is an open, global, multi-sector standard for efficient, accurate classification of products and services"}. Table~\ref{tab:unspsc} gives a summary of the levels in the taxonomy and its data. There are 4,302 items arranged into class, family, segment and commodity (lowest level). The {\em characteristic} column conveys the nature of abstraction across levels by reporting number of distinct (dissimilar) values, unique (count=1) values and their percentage, followed by highest frequency at a given level. 

% So, if the user inquires about a product, the chatbot can refer to the taxonomy to confirm what the user wants. As example,  a query on   {\em pliers} may refer to a surgical tool (Code: 42292303) or a vehicle servicing equipment (Code: 25191716) or a hand tool (Code: 27112106), and many variations therein. Thus, there can be a varieties strategies for a chatbot to help the user. It can go from highest level to lowest, or reverse, or ask randomly from the tree. Furthermore, if there is a restriction on how many turns the chatbot can take on this query, we want to explore if there are  querying strategies that are optimal.
 

% % Distinct means the number of dissimilar values contained for the selected attribute. Unique means the number and percentage of instances having a value for this attribute that no other instances have in the data.


% % ---------------------

% \begin{table}[t!]
% \scriptsize
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Level} & \textbf{Name} & \textbf{Characteristic} \\ \hline
% \textbf{4 - Highest} & Segment & 36; 3 (0\%); 825  \\ \hline
% \textbf{3} & Family & 173; 23 (1\%); 443  \\ \hline
% \textbf{2} & Class & 826; 216 (5\%); 49  \\ \hline
% \textbf{1 - Lowest} & Commodity & 4302; 4302 (100\%); 1  \\ \hline
% \end{tabular}
% \caption{Levels in UNSPSC Taxonomy.}
% \label{tab:unspsc}
% \end{table}
% % ---------------------

% % --------------------
% \subsection{Example 2 - Synthetic Domain of Information Retrieval}

% Conversational interface is considered especially suitable for feature or preference elicitation for at least two reasons~\cite{brennan1990conversation}. First, it is naturally interactive and thus users are more willing to provide additional information. Moreover, it can pro-actively and dynamically channel the information querying process in desired directions. 

% Suppose there are $m$ items described using
% $n$ features, $F_1$, .., $F_n$. To narrow down users' queries, previous work 
% has explored asking to confirm (Yes/No) clarification questions such as ``\textit{are you asking about topic X}''~\cite{horvitz1999computational}, and specify values for a feature by direct inquiry (e.g., ``\textit{What VALUE would you like for FEATURE X"}'')
% or multi-choice questions (e.g.``\textit{choices for FEATURE X are VALUE 1... VALUE N''})~\cite{chu2000mimic}. 
% We will assume that the features are binary. 
% The expected number of features that the user would report in answering a question is $\lambda_{NF}$, the recall rate of the NLP system is $R_{nlp}$, and each unknown feature's information gain is $IG$. 

% Such a setting can be used to model an online store selling shirts and trousers (i.e., items) to users. The features can be color, fabric and price category.  A person searching the store may have preferences about fabric and constraints about color when they are buying items together.

% --------------------
% \subsection{Example 3 - Navigating Alternative Choices}

% {\bf TO BE REMOVED BUT ELEMENTS INTRODUCED BACK IN 2nd EXAMPLE}

% Consider a simple conversation scenario related to route 
% advisory which suggests to a person best routes to take in a city. 
% A person, Max, lives in city which is laid
% out in a 4x4 grid as illustrated in Figure~\ref{fig:eg-travel}.
% His home is at location (1,1), office at (1,4), and there are two
% airports at (4,1) and (4,4). He has an agent, Angela, whom
% we want to design.

% For a given out-of-town travel, Max may want to go to a 
% specific airport starting from a location depending on his
% schedule for the day. A sample conversation strategy (Strategy 1)
% may be:

% \noindent{\bf Strategy 1:}
% \begin{enumerate}
% \item {\em Max: } Angela, what is the best way to go today to airport?
% \item {\em Angela: } Hi Max, is it the usual flight in morning from 
%     Home to JFK?
% \item {\em Max:} No, this is in evening.
% \item {\em Angela: } Ok. If your flight is from JFK in evening,
%      here is a route from office. ...
% \end{enumerate}

% A longer dialog strategy (Strategy 2) is to ask the user for each
% piece of information needed. 

% \noindent{\bf Strategy 2:}
% \begin{enumerate}
% \item {\em Max: } Angela, what is the best way to go today to airport?
% \item {\em Angela: } Hi Max, where will you leave from? 
% \item {\em Max: } It will be from office.
% \item {\em Angela: } Ok. Which airport do you want to go to? 
% \item {\em Max: } JFK
% \item {\em Angela: } What time will you like to go? 
% \item {\em Max: } In the evening.
% \item {\em Angela: } Ok. Here is a route from office to JFK ...
% \end{enumerate}

% Notice that Strategy-2 is longer than Strategy-1, imposing cognitive 
% load on the user. However, Strategy-1 relies on preferences
% that may or may not be valid in the on-going conversation.

% % -------------------------------------------------------------------

% \begin{figure}
%  \centering
%    \includegraphics[width=0.5\textwidth]{figs/eg-travel.jpg}
%   \caption{A simple route advisory task domain.}
%   \label{fig:eg-travel}
% \end{figure}
% % -------------------------------------------------------------------



% \begin{itemize}
% \item {\em Conversation Model:}
% \item {\em Task Model:}
% \item {\em Execution Model:}
% \end{itemize}

% % --------------------
% \subsection{Related Work}

% %% KRT: Cannot use below text, it is from the UISP paper
% % The planning community has also seen advances in the problems of measuring the distance between plans~\cite{roberts2014evaluating,goldman2015measuring}, and generating diverse plan alternatives~\cite{nguyen2012generating}. However, very little research has focused on exactly what the different metrics that go into creating diverse plans should be. ...

% Some references added.
 %\nocite{cranshaw2017calendar}

% --------------------


==> builders.tex <==
% --------------------
\section{Building Data-Consuming Chatbots}
\label{sec:builders}
% --------------------

% {\em Analogy with device independent or dependent application development}. 

% -----------------------------------------

\begin{figure}
 \centering
   \includegraphics[width=0.45\textwidth]{figs/chatbot-arch.jpg}
  \caption{The architecture of a data-driven chatbot.}
  \label{fig:chatbot-arch}
\end{figure}
% -----------------------------------------

The core problem in building chatbots is that of dialog management, i.e., creating dialog responses to user's utterances.
The system architecture of a typical data-consuming dialog manager  (DM) is shown in Figure~\ref{fig:chatbot-arch}. Given the user's utterance, it is analyzed to detect her intent and a 
policy for response is selected. This policy may call for querying a database, and the result is returned which is used by response generator to create a response using templates. The system can dynamically create one or more queries which involves selecting tables and attributes, filtering values and testing for conditions,  and assume defaults for missing values. It may also decide not to answer a request if it is unsure of a query's result correctness.

% Given a database, it is imperative to understand a user’s intent by parsing her query and provide accurate information that satisfy her goal in a timely manner.
% To achieve this, we need a dialog manager (DM) that can manage its conversation with the user and can search the database efficiently.


There are many approaches to tackle DM  in literature including finite-space, frame-based, inference-based and statistical learning-based \cite{chatbot-survey-statistical-ml,chatbot-book,minim-dialog,young2013pomdp} of which  finite-space and frame-based are most popular with mainstream developers. 
Task-oriented DMs  have traditionally been built using rules.
Further, a DM contains several independent modules which are optimized separately, relying on huge amount of human engineering 
(why end-to-end). 
The recent trend is to train DM from end-to-end, allowing error signal from the end output of DM to be back-propagated to raw input, so that the whole DM can be jointly optimized.

% Why learning: rule-based systems can be fragile


% \subsection{Why dialogs}
Considerations in exploring data with dialog:
\begin{itemize}
\item The data in a domain may consist of multiple tables, attributes (columns) and rows. The user utterance could lead to discovering them and they then become part of the context of query. (uncertainty exists in understanding users’ intents).
\item Natural order of user queries: Users have a cognitive order of asking to explore data, and that becomes shared context. (users’ cognitive process is dynamic)
\item Query execution is order dependent for cost reasons. Returning the full database dump is expensive. (manage cost)
\item Queries are in natural language v/s symbolic (formal) languages repositories support (relational, tree-based). (mappings between NLP and symbolic languages are imperfect)
\item There is a limit to the max number of turns, at the end of which, the system can give up. (diminishing return)

\end{itemize}
 
% Before:
% \begin{itemize}
% \item User needs knowledge of schema
% \item User needs knowledge of query language (SQL)
% \item System passively accepts user input 
% \item System may return large set of solutions and slowly
% \end{itemize}


% After:
% \begin{itemize}
% \item User does not need knowledge of database schema; only data types (columns/ slots)
% \item User does not need query language knowledge
% \item System will proactively prompt user towards efficient queries
% \item System can use query complexity to characterize dialog complexity

% \end{itemize}

To handle the issue of fairness, open data has  to be augmented.
Apart from standard information like data and size, most repositories also explain usage license (context), how data was obtained (provenance), semantics of missing values and units, and a responsible person. But the current metadata do not cover fairness considerations which many of their datasets will face, and this is where researchers have proposed to use data-sheets \cite{dataset-datasheets}. They can be used along with techniques in AI Fairness Toolkit\footnote{https://github.com/IBM/AIF360} to address issues of fairness and transparency with chatbots \cite{dialog-ethics} to build trust with users..

% --------------------



==> challenges.tex <==
% --------------------
\section{Technical Challenges}
\label{sec:prob}



% --------------------
\subsection{Incorporating Domain Knowledge and Learned Models}

% --------------------
\subsection{Interleaving Planning and Execution}


%DRAFT ADDED BELOW. BIPLAV, IS THIS WHAT YOU ARE EXPECTING?

A bounded-length planning problem is a structure
$\Pi = ({\cal V}, {\cal O}, s_0, k)$.
${\cal V}$ is a finite set of variables, where
each variable has a finite domain.
A complete state (shorter, a state) is a tuple where each variable
in ${\cal V}$ is instantiated to a value from its domain.
A tuple containing only a subset of instantiated variables
is called a partial state.
${\cal O}$ is a finite set of operators.
An operator $o \in {\cal O}$ has a precondition 
$\mathit{pre}(o)$, an effect $\mathit{eff}(o)$,
a cost $c(o)$ and an utility $r(o)$.
Preconditions and effects are partial states.
The cost and the utility are non-negative numbers.

[TODO: {\bf Biplav/Adi}: Discuss goals of dialog]

% {\bf Question for the team:}
% \emph{Should we define both a cost and a utility for the operators?
% In this case, we end up with multi-objective planning 
% (or multi-objective MDPs).}
% {\\ \bf Biplav: yes. }

There could be many possible objectives for dialog planning depending on applications.  
\begin{itemize}
\item O1: Minimize $\sum_l$ ${cost}_i$
\item O2: Maximize Net Benefit; $\sum_l$ (${utility}_i$ - ${cost}_i$)
\item O3: Maximize Discounted Net Benefit; $\sum_l$ (${utility}_i$ - ${cost}_i$) * $\gamma^i$

\end{itemize}


A partial state $s_1$ and a state $s_2$ are consistent
if their common variables have the same instantiation.
An operator $o$ is applicable in a state $s$
iff $\mathit{pre}(o)$ is consistent with $s$.
The result of applying $o$ to $s$ is a new state
$\gamma(s,o)$
that is consistent with $\mathit{eff}(o)$ and with
the partial state obtained from $s$ by removing
all the variables appearing in $\mathit{eff}(o)$.

The initial state $s_0$ is a complete state,
and $k$ is a positive integer.

A valid plan $o_1 \dots o_j$ is a sequence of operators such that:
i) $o_1$ is applicable in $s_0$, $o_2$ is applicable
in $\gamma(s_0,o_1)$ and so on; and
ii) the total number of operators $j$ does not exceed $k$.

{\bf Question for the team:}
{\emph {Do we handle contingent plans, or just sequential plans?}}

Observe that there is no notion of a goal state.
Any plan, including the empty plan, is a valid solution,
but plans may differ in their cost and utility.
The cost of a plan is the sum of the costs of all contained actions.
The utility of a plan is defined similarly.
When considering both criteria, our planning task is a multi-objective optimization problem.

[{\bf Radu}: Add POMDP connection, cite results]

{\bf Remark:}
\emph{Our plans look like finite-horizon policies,
where we try to maximize the reward within a finite horizon.
I wonder what related work does exist in MDPs.}

% ---------------------
\subsection{O1 - Cost Minimizing Dialogs}

\begin{itemize}
\item Constant cost
\end{itemize}

% ---------------------
\subsection{O2 - Net Benefit Maximizing Dialogs}

\begin{itemize}
\item Constant utility and cost
\item Varying utility and constant cost
\end{itemize}



% --------------------


==> discussion.tex <==
% --------------------
\section{Discussion}
\label{sec:disc}

Authors have created a chatbot to help with data analysis \cite{chatbot-data-analysis}. However, there is focus is on data analysts.

% --------------------



==> experiments.tex <==
% --------------------
\section{Experiments}
\label{sec:expts}

% --------------------



==> water.tex <==
% --------------------
\section{Decision-Support for Water Usage With a Multi-Modal Conversation Interface}
\label{sec:water-adv}

The global situation of water quality around the world is alarming in both developing and developed countries\cite{un-water} because water demand continues to rise while existing sources for fresh water are getting polluted. A key strategy for tackling  water pollution is engaging people. 
A person makes many daily decisions touching on water usage activities like for
 profession (e.g., fishing, irrigation, shipping), recreation (e.g, boating), wild life conservation (e.g., dolphins) or just regular living (e.g., drinking, bathing, washing). Accessible tools for public are particularly useful to handle public health challenges such as the Flint water crisis \cite{flint}. 
 
 A decision in this space needs to consider the activity (purpose) of the water use; relevant water quality parameters and their applicable regulatory standards for safety; available measurement technology, process, skills and costs; and actual data. 
 There are further complication factors: there may be overlapping regulations due to geography and administrative scope; one may have to account for alternative ways to measure a particular water quality parameter that evolves over time; and water data can have issues like missing values or at different levels of granularity. 
 The very few tools available today target water experts such as WaterLive mobile app for Australia \footnote{http://www.water.nsw.gov.au/realtime-data
},  Bath app for UK\footnote{2https://environment.data.gov.uk/bwq/profiles/}, and GangaWatch for India \cite{gw-demo} and assume technical understanding of sciences. 
% Accessible tools for public are particularly useful to handle public health challenges such as the Flint water crisis \cite{flint}. 

%  A further complication is that there may be missing data for a given location, time or parameters of interest; there may be overlapping regulations and there may be alternative ways to measure a particular water quality parameter.  
% Finally, end users need to understand the suggested advice given available data and not take it out of context. 


% -----------------------------------------

\begin{figure}
 \centering
   \includegraphics[width=0.45\textwidth]{figs/snap1.png}
  \caption{A screenshot of {\em Water Advisor}. See video of it in action at https://youtu.be/z4x44sxC3zA.}
  \label{fig:screen-shot-wa}
\end{figure}
% -----------------------------------------



% Nevertheless, given the importance of water decisions, it is surprising that there is an absence of decision support tools for general public. 


% ------
\subsection{Water Advisor}

Water Advisor (WA) is intended to be a  data-driven assistant that can guide people without requiring any special water expertise.  One can trigger it via a conversation to get an overview of water condition at a location, explore it by filtering and zooming on a map, and seek details on demand (Figure~\ref{fig:screen-shot-wa}) by exploring relevant regulations, data or other locations.
The current prototype uses water quality data available from Flint, MI\footnote{http://www.michigan.gov/flintwater/0,6092,7-345-76292\_76294\_76297---,00.html}
but future extensions will use open water data from US Geological Survey\footnote{https://waterdata.usgs.gov/nwis/current/?type=quality} (USGS) that is refreshed for thousands of places in US per day. However, the number of water quality parameters, for which data is available, varies widely between locations and over time, making generation of useful advice challenging. 
For regulations, WA relies on information provided by multiple agencies at national (US, India) and state levels (Michigan, New York), which has been consolidated for reuse\footnote{https://github.com/biplav-s/water-info}.


% ------
\subsection{Technical Issues}


% \noindent Chatbots, which can engage people in natural dialog conversation, have gained popularity recently drawn by numerous platforms to create them quickly for any domain. A broad class of such agents deal with answering a user's questions or providing them recommendations in a given domain. A  practical question that these dialogs raise is how well can an agent keep the person engaged and provide meaningful value, within a reasonable upper-bound on the number of dialogs in a conversation. 

%There are a few factors at play. 
In a water advising application, one or more users may need to interact with the chatbot if handling a complex decision like water contamination. 
The tool has to detect the user's information goals and meet them at lowest cognitive cost. The system uses a natural language classifier (NLC) to understand user utterance, and its error rate varies with input. The system has to decide whether to ask clarifying questions if it has low confidence and there are many ways to respond. The user may have preferences about how they specify an input (like location) and the kind of response 
they want (visual v/s textual). We discuss a range of issues below for exposition {\em but note that the current WA prototype handles only a subset of following integration issues}. 

% In summary, the factors are:
% \begin{itemize}
%     \item  Clarifying questions: user's information goals,
%          cost of questions; estimate of answers' utility
%     \item  NLC accuracy: discrete or continuous/ probabilistic 
%         accuracy of understanding user's inputs/ goals; clarifying
%         questions improve agent confidence
%     \item Recommendation engine: meta-features of solution space - 
%         number of candidate solutions, solution dimensions like 
%         cost
%     \item  User preference: over meta-features of solution space 
%          like goodness of solution, length
%     \item  Decision problem related: cost of action; 
%          estimate of action's failure to give intended result
% \end{itemize}    

\subsubsection{Learning} plays an important role in understanding user's utterance, finding reliable water data samples in the database based on region and duration of interest, discovering issues in water quality and improving overall performance over time. In the prototype, for utterances, we use trained user models from commercial systems and for water quality, a simple regression method. 


\subsubsection{Representation} is needed to map water's usage purpose to quality parameters  and model safe limits of pollution parameters with different mathematic properties (e.g., polarity). It also helps map water purpose to regulations and further, aggregate and reconcile the latter when a region falls under overlapping jurisdiction of regulations. We represent this as geographically-scoped attribute-value pair in JSON format and make it publicly available for others to use and extend\footnote{https://github.com/biplav-s/water-info}. 

\subsubsection{Reasoning} is crucial to keep conversation focused based on system usability goals and user needs.  One can model cognitive costs to user based on alternative system response choices and seek to optimize short-term and long-term behavior. Reasoning can further help to short-list regulations based on water activity and region of interest, generate advice and track explanations. We currently use rules on geographical scope and missing values to determine system response. 
 

\subsubsection{Execution} is autonomous as the agent can choose to act
by (a) asking clarifying questions about water usage goals or locations, (b) asking user's preference
about advice, (c) seeking most reliable water data for region and time interval of interest from available external data sources, and corresponding subset of compatible regulations (d) invoking reasoning to generate an advice for water usage using filtered water data and regulations, (e) visualizing and explaining its output using water regulations, and (f) using one or more suitable modalities available at any turn of user interaction, i.e., chat, maps and document views. 
The current prototype uses a simplistic  strategy for execution based on error rates, system confidence and usability rules.

\subsubsection{Human Usability Factors} have to be modeled and supported during WA's operation. In the current prototype, the user-interface controller module automatically keeps the different modalities synchronized so that the user is looking at consistent information across them. The system has to be aware of missing data or assumptions it is making, and needs to take them into account while communicating output advice in generated natural language.  One avenue for future exploration is to measure and track complexity of interaction \cite{dial-comp} and use sensed signals to pro-actively improve user experience. Another is to combine close-ended and open-ended questioning strategies for efficient interaction \cite{open-close-iui18}.

\subsubsection{Ethical Issues} can emerge whenever a piece of technology is used among people at large. In the context of conversations, a recent paper surveys ethical issues \cite{dialog-ethics} like biases, adversarial
examples, privacy violations, safety
challenges and reproducibility concerns. 
A water-use chatbot can conceivably create bias among users of different activity subgroups (e.g., preferring recreation over drinking), compromise on privacy of users who submit queries about an activity or a region, and create public safety concerns (e.g., when users find scarcity of good quality water). We have not considered them in the prototype, however.


% % --------------------
% \subsection{Decision-Support to Explore Exo-planets}

% \begin{figure*}
%  \centering
%    \includegraphics[width=0.7\textwidth]{figs/tyson-display.jpg}
%   \caption{Snapshot of display after interactions with agent. See video  of the demonstration at http://ibm.biz/tyson-demo}
%   \label{fig:view}
% \end{figure*}
% % -----------------------------------------


% --------------------

